CKConv: Continuous Kernel Convolution For Sequential Data

Conventional neural architectures for sequential data present important limitations. Recurrent networks suffer from exploding and vanishing gradients, small effective memory horizons, and must be trained sequentially. Convolutional networks are unable to handle sequences of unknown size and their memory horizon must be defined a priori. In this work, we show that all these problems can be solved by formulating convolutional kernels in CNNs as continuous functions. The resulting Continuous Kernel Convolution (CKConv) allows us to model arbitrarily long sequences in a parallel manner, within a single operation, and without relying on any form of recurrence. We show that Continuous Kernel Convolutional Networks (CKCNNs) obtain state-of-the-art results in multiple datasets, e.g., permuted MNIST, and, thanks to their continuous nature, are able to handle non-uniformly sampled datasets and irregularly-sampled data natively. CKCNNs match or perform better than neural ODEs designed for these purposes in a faster and simpler manner.

==> tables/appx-classification-1d.tex <==
\begin{table}
\centering
\vskip -2mm
\caption{Test accuracy on sMNIST, pMNIST, sCIFAR10 and npCIFAR10. \todo{Conclusions?}}
\label{tab:full-smnist}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{sMNIST} & \sc{pMNIST} & \sc{sCIFAR10} & \sc{npCIFAR10} \\
 \midrule
 DilRNN \citep{chang2017dilated} & 44\sc{k} & 98.0 & 96.1 & - & -\\
  IndRNN \citep{li2018independently} & 83\sc{k} & 99.0 & 96.0& - & - \\
  %LSTM \citep{bai2018empirical} &70\sc{k}& 87.2 & 85.7  & - \\
 %GRU \citep{bai2018empirical} &70\sc{k}&   96.2 & 87.3  & - \\
   TCN \citep{bai2018empirical} &70\sc{k}& 99.0 & 97.2  & - & - \\
  r-LSTM \citep{trinh2018learning} & 0.5\sc{m} & 98.4 & 95.2 & 72.2 & -\\
 Self-Att. \citep{trinh2018learning} &0.5\sc{m} & 98.9 & 97.9 & 62.2 & -\\
 TrellisNet \citep{bai2018trellis}& 8\sc{m} & 99.20 & 98.13 & 73.42 & - \\
 URLSTM \citep{gu2020improving} & - & 99.28 & 96.96 & 71.00 & - \\
  URGRU + Zoneout \citep{gu2020improving} & - & 99.27 & 96.51 & \textbf{74.40} & - \\
  HiPPO \citep{gu2020hippo} & 0.5\sc{m} & - & \textbf{98.30} & - & - \\
  Lipschitz RNN \citep{erichson2020lipschitz} & 158\sc{k} & 99.4 & 97.3 & 64.2 & 59.0 \\
  coRNN \citep{rusch2020coupled} & 134\sc{k} & \textbf{99.4} & 97.3 & - & 59.0 \\
  UnICORNN \citep{rusch2021unicornn} & 135\sc{k} & - & 98.4 & - & \textbf{62.4} \\
  pLMU \citep{chilkuri2021parallelizing} & 165\sc{k} & - & 98.49 & - & -\\
\midrule
CKCNN-2 & 98\sc{k} & 99.31 & 98.00 & 62.25 & 60.5\\
CKCNN-2-Big & 1\sc{m} & 99.32 & 98.54 & 63.74 & 62.2 \\
CKTCN$_{\text{\sc{Fourier}}}$-2 & \todo{...\sc{m}} & 99.44 & 98.40 & 68.28 & 66.26 \\
CKTCN$_{\text{\sc{Gabor}}}$-2 & \todo{...\sc{m}} & 99.52 & 98.38 & 69.26 & 67.52 \\
CKTCN$_{\text{\sc{MAGNet}}}$-2 & 105\sc{k} & \textbf{99.55} &\textbf{ 98.57} & \textbf{74.58} & \textbf{67.37} \\
\midrule
FlexTCN-2 & 108\sc{k} & \textbf{99.60} & \textbf{98.61} & \textbf{78.99} &  \textbf{67.11}\\
FlexTCN-4 &  241\sc{k} & \textbf{99.60} & \textbf{98.72} & \textbf{80.26} & \textbf{67.42}\\
FlexTCN-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\midrule
FlexTCN$_{\text{SIREN}}$-6 & \todo{...\sc{m}} & 99.03 & 95.36 & 69.24 & 57.27 \\
FlexTCN$_{\text{Fourier}}$-6 & \todo{...\sc{m}} & 99.49 & 97.97 & 74.79 & 67.35 \\
FlexTCN$_{\text{Gabor}}$-6 & \todo{...\sc{m}} &  99.50 & 98.37 & 78.36 & 67.56 \\
FlexTCN$_{\text{MAGNet}}$-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\bottomrule
\end{tabular}}
\end{small}
\end{table}

==> tables/appx-classification-cifar10.tex <==
\begin{table}%{r}{0.48\textwidth}
\centering
\caption{Full results on CIFAR-10. We report results over three runs per setting. CIFARResNet-44 w/ CKConv is a CIFARResNet-44 where all convolutional layers are replaced with CKConvs with $k = 3$. CIFARResNet-44 w/ FlexConv is a CIFARResNet-44 where all convolutional layers are replaced with FlexConv with learned kernel size, except for the shortcut connections of the strided convolutional layers, which are pointwise convolutions. *Results are taken from the respective original works instead of reproduced. \dagger Results are from single run.}
\label{tab:full-cifar-10}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{ccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} & \sc{CIFAR-10} \\
    & & \sc{Acc.} \\ \midrule
    DCN-$\sigma^{ji}$ \citep{tomen2021deep} & 0.47\sc{m} & 89.7 $\pm$ 0.3* \\
    N-Jet-CIFARResNet32 \citep{pintea2021resolution} & 0.52\sc{m} & 92.3 $\pm$ 0.3* \\
    N-Jet-ALLCNN \citep{pintea2021resolution} & 1.07\sc{m} & 92.5 $\pm$ 0.1* \\ \midrule
    CIFARResNet-44 \citep{he2016deep} & 0.66\sc{m} & 92.9*\!\dagger \\
    CIFARResNet-44 \citep{he2016deep} (our reproduction) & 0.66\sc{m} & 90.9 $\pm$ 0.2 \\\midrule
    CIFARResNet-44 w/ CKConv ($k = 3$) & 2.58\sc{m} & 86.1 $\pm$ 0.9 \\
    CIFARResNet-44 w/ FlexConv & 2.58\sc{m} & 81.6 $\pm$ 0.8 \\ \midrule
    FlexNet-7 w/ conv. ($k = 3$) & 0.17\sc{m} & 89.5 $\pm$ 0.3   \\
    FlexNet-7 w/ conv. ($k = 33$) & 20.0\sc{m} & 78.0 $\pm$ 0.3  \\
    FlexNet-7 w/ N-Jet \citep{pintea2021resolution} & 0.70\sc{m} & 91.7 $\pm$ 0.1  \\ \midrule
    \midrule
    CKCNN$_{\text{SIREN}}$-3 & 0.26\sc{m} & 72.4* \\ % 72.39
    CKCNN$_{\text{Fourier}}$-3 & 0.27\sc{m} & 83.8* \\ % 83.77
    CKCNN$_{\text{Gabor}}$-3 & 0.28\sc{m} & 85.6* \\ % 85.62
    CKCNN$_{\text{MAGNet}}$-3 & 0.28\sc{m} & 86.2* \\ % 86.18
    CKCNN-7 & 0.63\sc{m} & 71.7* \\ % 71.70
    CKCNN$_{\text{Fourier}}$-7 & 0.63\sc{m} & 84.6* \\ % 84.59
    CKCNN$_{\text{Gabor}}$-7 & 0.67\sc{m} & 87.7*  \\ % 87.65
    CKCNN$_{\text{MAGNet}}$-7 & 0.67\sc{m} & 85.9* \\ % 85.91
    \midrule
    FlexNet$_{\text{SIREN}}$-7 & 0.63\sc{m} & 88.9* \\ % 88.88
    FlexNet$_{\text{Fourier}}$-7 & 0.66\sc{m} & 91.6* \\ % 91.58
    FlexNet$_{\text{Gabor}}$-7 & 0.67\sc{m} & 92.0* \\ % 91.99
    \midrule
    FlexNet-3 & 0.27\sc{m} & 90.4 $\pm$ 0.2 \\
    FlexNet-5 & 0.44\sc{m} & 91.0 $\pm$ 0.5 \\
    FlexNet-7 & 0.67\sc{m} & 92.2 $\pm$ 0.1 \\
 \bottomrule
\end{tabular}}
% \end{sc}
% \end{small}
\end{center}
% \vspace{-5mm}
\end{table}

==> tables/classification-1d.tex <==
\begin{table}
\centering
\vskip -2mm
\caption{Test accuracy on sMNIST, pMNIST, sCIFAR10 and npCIFAR10. \todo{Conclusions.} \todo{Select models \& ablations to keep.} Tab.~\ref{tab:full-smnist} shows more results, including more baselines and ablations.}
\label{tab:smnist}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{sMNIST} & \sc{pMNIST} & \sc{sCIFAR10} & \sc{npCIFAR10} \\
 \midrule
 DilRNN & 44\sc{k} & 98.0 & 96.1 & - & -\\
  IndRNN & 83\sc{k} & 99.0 & 96.0& - & - \\
  %LSTM \citep{bai2018empirical} &70\sc{k}& 87.2 & 85.7  & - \\
 %GRU \citep{bai2018empirical} &70\sc{k}&   96.2 & 87.3  & - \\
   TCN &70\sc{k}& 99.0 & 97.2  & - & - \\
  r-LSTM & 0.5\sc{m} & 98.4 & 95.2 & 72.2 & -\\
 Self-Att. &0.5\sc{m} & 98.9 & 97.9 & 62.2 & -\\
 TrellisNet & 8\sc{m} & 99.20 & 98.13 & 73.42 & - \\
 URLSTM & - & 99.28 & 96.96 & 71.00 & - \\
  URGRU + Zoneout  & - & 99.27 & 96.51 & 74.40 & - \\
  HiPPO & 0.5\sc{m} & - & 98.30 & - & - \\
  Lipschitz RNN & 158\sc{k} & 99.4 & 97.3 & 64.2 & 59.0 \\
  coRNN & 134\sc{k} & 99.4 & 97.3 & - & 59.0 \\
  UnICORNN & 135\sc{k} & - & 98.4 & - & 62.4 \\
  pLMU  & 165\sc{k} & - & 98.49 & - & -\\
\midrule
CKCNN-2 & 98\sc{k} & 99.31 & 98.00 & 62.25 & 60.5\\
CKCNN-2-Big & 1\sc{m} & 99.32 & 98.54 & 63.74 & 62.2 \\
CKTCN$_{\text{\sc{Fourier}}}$-2 & & 99.44 & 98.40 & 68.28 & 66.26 \\
CKTCN$_{\text{\sc{Gabor}}}$-2 & & 99.52 & 98.38 & 69.26 & 67.52 \\
CKTCN$_{\text{\sc{MAGNet}}}$-2 & 105\sc{k} & 99.55 & 98.57 & 74.58 & 67.37 \\
\midrule
FlexTCN-2 & 108\sc{k} & 99.60 & 98.61 & 78.99 & 67.11\\
FlexTCN-4 &  241\sc{k} & 99.60 & \textbf{98.72} & 80.26 & 67.42\\
FlexTCN-6 & 375\sc{k} & \textbf{99.62} &  98.63 & \textbf{80.82} & \textbf{69.87} \\
\midrule
\midrule
FlexTCN$_{\text{SIREN}}$-6 &  & 99.03 & 95.36 & 69.24 & 57.27 \\
FlexTCN$_{\text{Fourier}}$-6 & & 99.49 & 97.97 & 74.79 & 67.35 \\
FlexTCN$_{\text{Gabor}}$-6 & &  99.50 & 98.37 & 78.36 & 67.56 \\
FlexTCN$_{\text{MAGNet}}$-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\bottomrule
\end{tabular}}
\end{small}
\end{table}

% DilRNN \citep{chang2017dilated}, 
% IndRNN \citep{li2018independently}, 
% TCN \citep{bai2018empirical}, 
% r-LSTM \citep{trinh2018learning}, 
% Self-Att. \citep{trinh2018learning}, 
% TrellisNet \citep{bai2018trellis}, 
% URLSTM \citep{gu2020improving}, 
% URGRU + Zoneout \citep{gu2020improving}, 
% HiPPO \citep{gu2020hippo}, 
% Lipschitz RNN \citep{erichson2020lipschitz}, 
% coRNN \citep{rusch2020coupled}, 
% UnICORNN \citep{rusch2021unicornn} and
% pLMU \citep{chilkuri2021parallelizing}.

==> tables/classification-cifar10.tex <==
\begin{table}
% \begin{wraptable}{r}{0.45\textwidth}
\vspace{-0mm}
\centering
\caption{Results on CIFAR-10. FlexNet is competitive with CIFARResNets and other learnable kernel size works. The FlexConv mask and MAGNet both improve over the baseline CKConv methods. We report results over three runs per setting. Time is reported as seconds per epoch of a converged model. Tab.~\ref{tab:full-cifar-10} shows more results, including more ablations. *Results are taken from the respective original works instead of reproduced. \!\dagger Results are from single run.}
\label{tab:cifar-10}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} & \sc{CIFAR-10} & \multirow{2}{*}{\sc{Time}} \\
    & & \sc{Acc.} & \\ \midrule
    CIFARResNet-44 & 0.66\sc{m} & 92.9*\!\dagger & - \\ \midrule
    DCN-$\sigma^{ji}$ & 0.47\sc{m} & 89.7 $\pm$ 0.3* & - \\
    N-Jet-CIFARResNet32 & 0.52\sc{m} & 92.3 $\pm$ 0.3* & - \\
    N-Jet-ALLCNN & 1.07\sc{m} & 92.5 $\pm$ 0.1* & - \\ \midrule
    FlexNet-7 w/ conv. ($k = 3$) & 0.17\sc{m} & 89.5 $\pm$ 0.3 & 41s   \\
    FlexNet-7 w/ conv. ($k = 33$) & 20.0\sc{m} & 78.0 $\pm$ 0.3 & 242s  \\
    FlexNet-7 w/ N-Jet & 0.70\sc{m} & 91.7 $\pm$ 0.1 & 409s  \\ \midrule
    % \midrule
    CKCNN-7 & 0.63\sc{m} & 71.7* & 266s \\ % 71.70
    CKCNN$_{\text{Gabor}}$-7 & 0.67\sc{m} & 87.6* & \todo{69s} \\ % 87.65
    CKCNN$_{\text{MAGNet}}$-7 & 0.67\sc{m} &  85.9* & 299s \\ % 85.91
    \midrule
    FlexNet$_{\text{SIREN}}$-7 & 0.63\sc{m} & 88.9* & 105s \\ % 88.88
    FlexNet$_{\text{Gabor}}$-7 & 0.67\sc{m} & 92.0* & 178s \\ % 91.99
    \midrule
    FlexNet-7 & 0.67\sc{m} & 92.2 $\pm$ 0.1 & 166s \\
 \bottomrule
\end{tabular}}
% \end{sc}
% \end{small}
\end{center}
\vspace{-7mm}
\end{table}
% \end{wraptable}

==> tables/classification-imagenet32.tex <==
\begin{table}
% \begin{wraptable}{r}{0.45\textwidth}
\vspace{0mm}
\centering
\caption{Results on ImageNet-32. *Results are taken from the respective original works instead of reproduced. \dagger Results are from a single run.}
\label{tab:imagenet-32}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} &  \multicolumn{2}{c}{\sc{ImageNet-32}} \\
    & & \sc{Top-1} & \sc{Top-5} \\ \midrule
    CIFARResNet-32 & 0.53\sc{m} & 26.41 $\pm$ 0.13 & 49.37 $\pm$ 0.15 \\ 
    WRN-28-1 & 0.44\sc{m} & 32.03*\!\dagger & 57.51*\!\dagger \\ \midrule
    FlexNet-5 & 0.44\sc{m} & 24.9 $\pm$ 0.4 & 47.7 $\pm$ 0.6 \\
  \bottomrule
\end{tabular}}
% \end{sc}
% \end{small}
\end{center}
\vspace{-5mm}
% \end{wraptable}
\end{table}

==> tables/classification-sequences.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\vspace{-5mm}
\vskip -2mm
\caption{Test accuracy on Character Trajectory, Speech Commands, Speech Commands Raw. \todo{Conclusions.}}
\label{tab:time-series}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{CT} & \sc{SC} & \sc{SC\_raw} \\
\midrule
GRU-ODE & 89\sc{k} & 96.2 & 44.8 & $\sim$10.0 \\
GRU-$\Delta t$ & 89\sc{k} & 97.8 & 20.0 & $\sim$10.0 \\
GRU-D & 89\sc{k} & 95.9 & 23.9 & $\sim$10.0 \\
ODE-RNN & 89\sc{k} & 97.1 & 93.2 & $\sim$10.0 \\
NCDE  & 89\sc{k} & 98.8 & 88.5 & $\sim$10.0 \\
\midrule
CKCNN & 100\sc{k} &\textbf{ 99.53 }& 95.27 & 71.66 \\
CKTCN$_{\text{Fourier}}$ & & - & 95.65 & 74.90 \\
CKTCN$_{\text{Gabor}}$ &  & - & 96.66 &  78.10 \\
CKTCN$_{\text{MAGNet}}$ & 105\sc{k} &  \textbf{99.53} & \textbf{97.01} & \textbf{80.69} \\
\midrule
FlexTCN-2 & 105\sc{sk} & \textbf{99.53} & \textbf{97.10} & \textbf{88.03}  \\
FlexTCN-4 & 239\sc{k} & \textbf{99.53} & \textbf{97.73} & \textbf{90.45}   \\
FlexTCN-6 & 373\sc{k} & \textbf{99.53} & \textbf{97.67} & \textbf{91.73} \\
\midrule
FlexTCN$_{\text{SIREN}}$-6 &  & - & 95.83 & \\
FlexTCN$_{\text{Fourier}}$-6 & & - & 97.62 &  \\
FlexTCN$_{\text{Gabor}}$-6 & & - & 97.35 & \\
FlexTCN$_{\text{MAGNet}}$-6 & 373\sc{k} & - & \textbf{97.67} & \textbf{91.73} \\
\bottomrule
\end{tabular}}
\end{small}
\vspace{5mm}
\end{wraptable}

==> tables/crossres-cifar10.tex <==
\begin{table}

\begin{minipage}{0.50\textwidth}
\vspace{8mm}
\centering
\caption{Results for alias-free FlexNets on \todo{CIFAR-10}.
% FlexNets reduce the accuracy gap at upscaling more than all other methods. We train each model for 100 epochs at resolution $16 \times 16$, then evaluate it at resolution $32 \times 32$. We report results over three runs per setting.
}
\label{tab:crossres}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} & \multicolumn{2}{c}{\sc{CIFAR-10 Acc.}} \\
    & & 16 px & $\Delta_{16 \textrm{px}}$ 32 px \\ \midrule % & fine-tuned \\ \midrule
    CIFARResNet-44 & 0.66\sc{m} & 85.8 $\pm$ 0.2 & -31.6 $\pm$ 1.3 \\ \midrule
    % 85.4 $\pm$ 0.3 & -31.2 $\pm$ 2.8 \\ \midrule % & 92.6 $\pm$ 0.2 \\ \midrule
    FlexNet-7 w/ conv. ($k = 3$) & 0.17\sc{m} & 85.3 $\pm$ 0.2 & -21.2 $\pm$ 1.0 \\ % & \textbf{90.1} $\pm$ 0.1  \\
    FlexNet-7 w/ conv. ($k = 33$) & 20.0\sc{m} & 67.7 $\pm$ 0.6 & -57.1 $\pm$ 1.6 \\ % & 79.2 $\pm$ 0.4  \\
    FlexNet-7 w/ N-Jets & 0.70\sc{m} & \textbf{86.4} $\pm$ 0.2 & -5.5 $\pm$ 1.3 \\ \midrule % & 89.5 $\pm$ 0.1  \\ \midrule
    CKCNN-7$_{\textrm{SIREN}}$ & 0.63\sc{m} & 45.9 $\pm$ 1.0 & -15.8 $\pm$ 1.2 \\
    FlexNet-7$_{\textrm{SIREN}}$ & 0.63\sc{m} & 70.4 $\pm$ 0.8 & -50.0 $\pm$ 16.9 \\ \midrule
    FlexNet-7 w/o reg. & 0.67\sc{m} & \textbf{86.4} $\pm$ 0.4 & -34.4 $\pm$ 14.3 \\ \midrule % & 88.8 $\pm$ 0.6 \\ \midrule
    FlexNet-7 w/ reg. $f^+_{\textrm{MAGNet}}$ & 0.67\sc{m} & \textbf{86.5} $\pm$ 0.1 & -3.8 $\pm$ 2.0 \\ % & 89.0 $\pm$ 0.3  \\
    FlexNet-7 w/ reg. $f^+_{\textrm{FlexConv}}$ & 0.67\sc{m} & 85.1 $\pm$ 0.3 & \textbf{-3.3} $\pm$ 0.3 \\ % & 87.6 $\pm$ 0.2 \\
 \bottomrule
\end{tabular}}
\end{center}
% \vspace{-5mm}
\end{minipage}\hspace{5mm}
\end{table}

==> tables/crossres-imagenet-k.tex <==
\begin{table}
\centering
\caption{Results for alias-free FlexNets on CIFAR-10 and ImageNet-$\mathrm{k}$. $\Delta$ denotes difference in accuracy. 
% N-Jets and FlexConv perform comparatively bad on ImageNet-32. We train each model for 100 epochs on ImageNet-16, then evaluate on ImageNet-32. We report results over three runs per setting.
}
\label{tab:crossres-imagenet}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.75}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} &  \multicolumn{2}{c}{\sc{ImageNet-k Top-1}} \\
    & & $k = 16$ & $\Delta_{k = 16}$ $k = 32$ \\ \midrule % & fine-tuned \\ \midrule
    CIFARResNet-32 & 0.52\sc{m} & 16.1 $\pm$ 0.0 & -11.6 $\pm$ 0.4 \\ \midrule % \todo{RUNNING} \\ \midrule
    FlexNet-5 w/ N-Jets & 0.46\sc{m} & 15.7 $\pm$ 0.1 & -1.9 $\pm$ 0.4 \\ \midrule % & \todo{RUNNING}  \\ \midrule
    FlexNet-5 & 0.44\sc{m} & 14.9 $\pm$ 0.1 & -1.9 $\pm$ 1.7 \\ % & 24.8 $\pm$ 0.2 \\
 \bottomrule
\end{tabular}}
\end{center}
% \vspace{-5mm}
\end{table}
